StoryAnalogy: Deriving Story-level Analogies from Large Language Models to Unlock Analogical Understanding

Analogy-making between narratives is crucial for human reasoning. In this paper, we evaluate the ability to identify and generate analogies by constructing a first-of-its-kind large-scale story-level analogy corpus, \textsc{StoryAnalogy}, which contains 24K story pairs from diverse domains with human annotations on two similarities from the extended Structure-Mapping Theory. We design a set of tests on \textsc{StoryAnalogy}, presenting the first evaluation of story-level analogy identification and generation. Interestingly, we find that the analogy identification tasks are incredibly difficult not only for sentence embedding models but also for the recent large language models (LLMs) such as ChatGPT and LLaMa. ChatGPT, for example, only achieved around 30% accuracy in multiple-choice questions (compared to over 85% accuracy for humans). Furthermore, we observe that the data in \textsc{StoryAnalogy} can improve the quality of analogy generation in LLMs, where a fine-tuned FlanT5-xxl model achieves comparable performance to zero-shot ChatGPT.

==> floats/corr-results-cl.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\begin{tabular}{lcccccc}
\hline
                       & \multicolumn{3}{c}{\textbf{ProPara}} & \multicolumn{3}{c}{\textbf{ROCStories}} \\ \cline{2-7} 
\multicolumn{1}{c}{}   & R          & R-E        & R/E        & R           & R-E         & R/E         \\ \hline
\end{tabular}
\caption{{\color{red} Replace this with a figure. }}
\label{tab:corr-result-cl}

\end{table}


==> floats/corr-results-llms.tex <==
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc|rrrr|rrrr|rrrr|rrrr}
\hline
\multirow{2}{*}{}            & \multirow{2}{*}{\textbf{Instr.}} & \multirow{2}{*}{\textbf{n examples}} & \multicolumn{4}{c|}{ProPara}                                                                           & \multicolumn{4}{c|}{ROCStories}                                                                        & \multicolumn{4}{c|}{Word-Analogy}                                                                      & \multicolumn{4}{c}{ConceptNet}                                                                        \\ \cline{4-19} 
                             &                                  &                                      & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c|}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c|}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c|}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c}{R/E} \\ \hline
Random                       & \multicolumn{1}{l}{}             & \multicolumn{1}{l|}{}                & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} \\ \hline
\multirow{6}{*}{FlanT5-XXL}  & \multirow{3}{*}{Short}           & 0                                    & 44.1                    & 18.4                    & 4.1                     & 3.4                      & 7.2                     & -2.6                    & 3.9                     & -0.0                     & 40.1                    & 28.3                    & 12.2                    & 10.3                     & 36.3                    & 23.6                    & 5.3                     & 5.1                     \\
                             &                                  & 1                                    & 43.4                    & 17.9                    & 4.7                     & 3.3                      & 5.0                     & -6.2                    & -1.4                    & -4.3                     & 41.7                    & 30.2                    & 9.9                     & 10.3                     & 36.1                    & 26.0                    & 3.2                     & 4.8                     \\
                             &                                  & 3                                    & 41.1                    & 14.9                    & -1.4                    & -1.4                     & 2.4                     & -9.1                    & 0.7                     & -3.4                     & 40.2                    & 27.4                    & 6.5                     & 5.6                      & 38.3                    & 25.3                    & 5.7                     & 5.7                     \\ \cline{2-19} 
                             & \multirow{3}{*}{Long}            & 0                                    & 41.2                    & 19.7                    & -1.5                    & -2.5                     & 6.3                     & -5.1                    & -2.9                    & -6.2                     & 37.8                    & 29.6                    & 10.0                    & 9.3                      & 35.3                    & 27.9                    & 7.3                     & 9.6                     \\
                             &                                  & 1                                    & 41.7                    & 23.1                    & 0.5                     & 1.8                      & 7.4                     & -4.7                    & 3.9                     & 0.4                      & 38.5                    & 30.1                    & 3.0                     & 6.3                      & 39.2                    & 27.7                    & 9.3                     & 9.3                     \\
                             &                                  & 3                                    & 41.9                    & 21.8                    & 1.8                     & 4.8                      & 9.4                     & -8.7                    & 2.6                     & -2.4                     & 40.0                    & 27.5                    & 9.1                     & 8.3                      & 37.7                    & 26.7                    & 6.5                     & 8.1                     \\ \hline
\multirow{6}{*}{Llama-65B}   & \multirow{3}{*}{Short}           & 0                                    & -3.1                    & -1.5                    & 5.7                     & 6.0                      & -6.3                    & -5.6                    & 2.2                     & 0.4                      & -0.6                    & -7.5                    & 0.1                     & -3.1                     & 3.4                     & -4.8                    & 1.4                     & -1.8                    \\
                             &                                  & 1                                    & 15.7                    & 9.0                     & -0.6                    & -2.5                     & -1.8                    & 2.0                     & 9.7                     & 8.8                      & 24.9                    & 21.1                    & -0.2                    & 2.0                      & 25.9                    & 20.3                    & 7.6                     & 7.7                     \\
                             &                                  & 3                                    & 15.0                    & 5.5                     & -4.8                    & -3.4                     & -3.3                    & -10.2                   & -7.7                    & -9.9                     & 30.3                    & 15.2                    & 1.3                     & 3.3                      & 10.5                    & 22.6                    & -1.4                    & 7.8                     \\ \cline{2-19} 
                             & \multirow{3}{*}{Long}            & 0                                    & 2.5                     & 1.1                     & -6.0                    & -5.6                     & -2.0                    & 5.7                     & 0.6                     & 1.5                      & -2.2                    & nan                     & 4.0                     & 4.8                      & -1.2                    & 4.4                     & 1.2                     & 1.3                     \\
                             &                                  & 1                                    & 15.3                    & 16.6                    & 7.0                     & 7.3                      & 5.6                     & 1.0                     & 13.2                    & 11.0                     & 16.8                    & 26.5                    & -7.3                    & -0.1                     & 29.5                    & 24.1                    & 7.0                     & 6.9                     \\
                             &                                  & 3                                    & 16.8                    & 3.8                     & -1.7                    & -1.3                     & 0.4                     & -10.2                   & -3.4                    & -7.7                     & 31.6                    & 25.3                    & 5.9                     & 9.5                      & 13.8                    & 22.1                    & -5.1                    & 4.2                     \\ \hline
\multirow{6}{*}{GPT-3} & \multirow{3}{*}{Short}           & 0                                    & 31.3                    & 6.9                     & 1.0                     & -3.2                     & -0.3                    & -7.7                    & -0.9                    & -2.7                     & 39.0                    & 29.5                    & -9.9                    & 0.4                      & 36.0                    & 21.3                    & -4.7                    & 1.7                     \\
                             &                                  & 1                                    & 28.2                    & 12.9                    & -7.7                    & -5.9                     & 0.4                     & -13.1                   & -8.0                    & -10.6                    & 37.4                    & 25.5                    & 2.7                     & 5.9                      & 34.0                    & 18.5                    & -4.7                    & 0.3                     \\
                             &                                  & 3                                    & 20.3                    & 12.7                    & -13.6                   & -7.9                     & -2.5                    & -4.7                    & -5.9                    & -5.0                     & 30.0                    & 23.6                    & -4.0                    & -0.1                     & 23.0                    & 29.4                    & -7.7                    & 5.5                     \\ \cline{2-19} 
                             & \multirow{3}{*}{Long}            & 0                                    & 27.6                    & 5.0                     & -8.8                    & -7.9                     & 4.2                     & -5.5                    & 5.4                     & 2.8                      & 41.4                    & 26.7                    & 0.5                     & 4.3                      & 37.6                    & 15.8                    & -7.6                    & -2.3                    \\
                             &                                  & 1                                    & 27.0                    & 11.7                    & -1.7                    & -1.0                     & 2.1                     & -7.1                    & -1.5                    & -4.9                     & 39.0                    & 27.4                    & 3.5                     & 5.6                      & 35.0                    & 18.5                    & 4.6                     & 2.7                     \\
                             &                                  & 3                                    & 24.1                    & 11.4                    & -11.4                   & -6.4                     & -3.2                    & -2.8                    & -7.1                    & -6.4                     & 34.2                    & 26.9                    & 8.4                     & 8.6                      & 28.8                    & 30.0                    & 0.3                     & 7.9                     \\ \hline
\multirow{6}{*}{ChatGPT}     & \multirow{3}{*}{Short}           & 0                                    & 32.1                    & 13.1                    & 0.4                     & -1.7                     & 7.8                     & 0.6                     & 12.5                    & 7.6                      & 53.0                    & 40.1                    & 10.3                    & 12.0                     & 39.2                    & 31.3                    & 6.3                     & 9.7                     \\
                             &                                  & 1                                    & 29.6                    & 13.0                    & -1.0                    & -2.0                     & 3.8                     & 0.3                     & 6.6                     & 4.4                      & 49.2                    & 36.5                    & 16.0                    & 18.8                     & 42.8                    & 31.5                    & 4.9                     & 6.1                     \\
                             &                                  & 3                                    & 26.0                    & 18.2                    & 2.9                     & 5.2                      & 1.0                     & -1.9                    & -2.7                    & -4.3                     & 46.7                    & 28.4                    & -2.6                    & -3.9                     & 38.3                    & 28.2                    & -1.1                    & 1.3                     \\ \cline{2-19} 
                             & \multirow{3}{*}{Long}            & 0                                    & 35.2                    & 15.2                    & 0.2                     & -2.4                     & 10.0                    & -4.5                    & -4.9                    & -8.7                     & 53.3                    & 37.8                    & 10.6                    & 10.7                     & 44.4                    & 37.3                    & 6.2                     & 14.9                    \\
                             &                                  & 1                                    & 32.0                    & 14.1                    & -2.7                    & -3.3                     & 4.3                     & 1.6                     & 8.9                     & 6.6                      & 49.6                    & 33.1                    & 4.8                     & 5.4                      & 40.1                    & 34.0                    & 7.6                     & 12.7                    \\
                             &                                  & 3                                    & 26.9                    & 11.9                    & -5.0                    & -2.3                     & 1.7                     & -4.4                    & -0.3                    & -5.0                     & 46.6                    & 31.4                    & 4.6                     & 3.4                      & 32.1                    & 36.4                    & -2.5                    & 13.1                    \\ \hline
Human                        & \multicolumn{1}{l}{}             & \multicolumn{1}{l|}{}                & 54.9                    & 64.6                    & 66.9                    & 67.9                     & 82.9                    & 70.1                    & 56.5                    & 55.2                     & 67.1                    & 69.4                    & 77.0                    & 58.3                     & 53.7                    & 75.5                    & 72.6                    & 68.5                    \\ \hline
\end{tabular}
}
\caption{Spearman's r value (\%). STS-style evaluation on \datasetname. 
Here E, R, R-E, and R/E corresponds to \entsim, \relsim, \texttt{RelSim-EntSim}, and \texttt{RelSim/EntSim}, respectively.}
\label{tab:corr-result-llm}

\end{table*}

==> floats/corr-results.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llllllllllllllll|llll}
\hline
            & \multicolumn{4}{c}{\textbf{ProPara}}                                                                  & \multicolumn{4}{c}{\textbf{ROCStories}}                                                               & \multicolumn{4}{c}{\textbf{Word-Analogy}}                                                             & \multicolumn{4}{c|}{\textbf{ConceptNet}}                                                               & \multicolumn{4}{c}{\textbf{All}}                                                                      \\ \cline{2-21} 
            & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c|}{R/E} & \multicolumn{1}{c}{E}   & \multicolumn{1}{c}{R}   & \multicolumn{1}{c}{R-E} & \multicolumn{1}{c}{R/E} \\ \hline
Random      & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.0} \\ \hline
RoBERTa     & 45.2                    & 41.9                    & 6.0                     & 6.2                     & 20.6                    & 22.2                    & 3.6                     & 7.6                     & 34.8                    & 24.5                    & -6.4                    & 0.9                     & 34.9                    & 28.8                    & 1.9                     & 9.8                      & 33.9                    & 29.4                    & 1.3                     & 6.1                     \\
SimCSE      & 48.0                    & 38.4                    & 1.2                     & 1.8                     & 14.4                    & 12.7                    & -0.5                    & 2.6                     & 43.2                    & 26.8                    & -10.7                   & -2.0                    & 30.7                    & 21.2                    & -3.1                    & 3.7                      & 34.1                    & 24.8                    & -3.3                    & 1.5                     \\
OpenAI-ada  & 52.8                    & 43.9                    & 3.4                     & 3.4                     & 22.3                    & 21.7                    & 0.0                     & 4.5                     & 41.3                    & 24.0                    & -11.8                   & -3.8                    & 32.3                    & 17.8                    & -7.6                    & -1.2                     & 37.2                    & 26.9                    & -4.0                    & 0.7                     \\ \hline
DMR         & 34.8                    & 42.0                    & 13.4                    & 12.6                    & 20.1                    & 35.0                    & 14.9                    & 20.1                    & 17.3                    & 18.7                    & 3.7                     & 7.3                     & 21.9                    & 19.1                    & 1.2                     & 5.5                      & 23.5                    & 28.7                    & 8.3                     & 11.4                    \\
GloVe-Noun  & 35.2                    & 18.5                    & -7.9                    & -7.8                    & 9.4                     & 6.9                     & 1.6                     & 2.5                     & 29.8                    & 14.2                    & -11.0                   & -5.6                    & 27.7                    & 13.0                    & -8.2                    & -2.2                     & 25.5                    & 13.2                    & -6.4                    & -3.3                    \\
GloVe-Verb  & 27.3                    & 44.8                    & 22.1                    & 21.3                    & 22.7                    & 34.2                    & 12.3                    & 17.3                    & 9.6                     & 7.0                     & -1.0                    & 1.3                     & 13.0                    & 1.0                     & -8.5                    & -7.2                     & 18.1                    & 21.7                    & 6.2                     & 8.2                     \\
GloVe-All   & 36.3                    & 29.0                    & -0.6                    & -1.0                    & 28.7                    & 27.2                    & -0.5                    & 4.8                     & 26.1                    & 12.3                    & -10.2                   & -5.1                    & 18.6                    & 3.3                     & -12.0                   & -7.9                     & 27.4                    & 18.0                    & -5.8                    & -2.3                    \\
RelBERT     & 37.9                    & 38.8                    & 7.7                     & 7.5                     & 15.6                    & 20.6                    & 6.0                     & 9.1                     & 28.6                    & 15.5                    & -9.5                    & -3.6                    & 26.6                    & 24.7                    & 1.7                     & 8.2                      & 27.2                    & 24.9                    & 1.5                     & 5.3                     \\ \hline
FlanT5-xxl  & 41.9                    & 21.8                    & 1.8                     & 4.8                     & 9.4                     & -8.7                    & 2.6                     & -2.4                    & 40.0                    & 27.5                    & 9.1                     & 8.3                     & 37.7                    & 26.7                    & 6.5                     & 8.1                      & 32.3                    & 16.8                    & 5.0                     & 4.7                     \\
LLaMa-65B   & 16.8                    & 3.8                     & -1.7                    & -1.3                    & 0.4                     & -10.2                   & -3.4                    & -7.7                    & 31.6                    & 25.3                    & 5.9                     & 9.5                     & 13.8                    & 22.1                    & -5.1                    & 4.2                      & 15.6                    & 10.3                    & -1.1                    & 1.2                     \\
GPT-3.5     & 24.1                    & 11.4                    & -11.4                   & -6.4                    & -3.2                    & -2.8                    & -7.1                    & -6.4                    & 34.2                    & 26.9                    & 8.4                     & 8.6                     & 28.8                    & 30.0                    & 0.3                     & 7.9                      & 21.0                    & 16.4                    & -2.5                    & 0.9                     \\
ChatGPT     & 26.9                    & 11.9                    & -5.0                    & -2.3                    & 1.7                     & -4.4                    & -0.3                    & -5.0                    & 46.6                    & 31.4                    & 4.6                     & 3.4                     & 32.1                    & 36.4                    & -2.5                    & 13.1                     & 26.8                    & 18.8                    & -0.8                    & 2.3                     \\ \hline
RoBERTa-Reg & 38.9                    & 41.5                    & 25.2                    & 27.1                    & 14.6                    & 28.0                    & 11.0                    & 15.3                    & 26.0                    & 34.2                    & 21.8                    & 25.3                    & 16.9                    & 25.3                    & 11.5                    & 17.4                     & 24.1                    & 32.3                    & 17.4                    & 21.3                    \\
RoBERTa-CL  & 38.2                    & 63.9                    & 26.8                    & 27.3                    & 34.0                    & 61.2                    & 30.1                    & 37.9                    & 40.5                    & 45.0                    & 11.8                    & 21.0                    & 30.9                    & 38.2                    & 12.4                    & 22.3                     & 35.9                    & 52.1                    & 20.3                    & 27.2                    \\ \hline
Human       & 54.9                    & 64.6                    & 66.9                    & 67.9                    & 82.9                    & 70.1                    & 56.5                    & 55.2                    & 67.1                    & 69.4                    & 77.0                    & 58.3                    & 53.7                    & 75.5                    & 72.6                    & 68.5                     & 64.7                    & 69.9                    & 68.3                    & 62.5                    \\ \hline
\end{tabular}
}
\caption{Spearman's r value (\%). STS-style evaluation on \datasetname. 
Here R, R-E, and R/E corresponds to the different definition of analogy scores \texttt{RelSim}, \texttt{RelSim-EntSim}, and \texttt{RelSim/EntSim}, respectively. 
Here, the LLM performance are under the ``long instruction+3-shot'' setting.}
\label{tab:corr-result-succinct}

\end{table*}




==> sections/extra-experiments.tex <==




\section{Experiments}
With the annotation data, we look into the following research questions (RQs):
\begin{itemize}
    \item RQ1: Are current language model embeddings effective for story analogy retrieval? If not, can we define a feature-engineering-free model that generates reliable embeddings for modeling relational similarities?
    \item RQ2: How are current LMs performing to generate analogies? Can smaller language models generate satisfactory analogous stories with / without finetuning?
    \item RQ3: Can we retrieve analogous stories for innovative problem solving?
\end{itemize}

We then conduct experiments on the following three settings to answer the above research questions.
% \subsection{Task formulation}
\begin{itemize}
    \item \textbf{Analogy retrieval.} Retrieving analogous texts from a big corpus. How do current methods (e.g. LLMs embeddings) perform on analogy retrieval?
    \item \textbf{Analogy generation.} Can current language models do well in generating analogies? Moreover, can they benefit from the proposed data? (e.g. Small LMs generate high quality analogies after finetuning?)
    \item \textbf{Problem solving by analogy retrieval.} \citet{webb2022emergent} found that after providing an analogous story to GPT-3.5, it can found appropriate solutions to questions. 
\end{itemize}

\subsection{Analogy retrieval}

\subsubsection{Unsupervised evaluation of analogy retrieval}


\begin{itemize}
    \item Random \& Human performance.
    \item LM embeddings + Cosine similarity. (Vanilla LMs, SimCSE variants, GPT-3.5 embedding text-embedding-ada-003)
    \item GPT-3.5-gen (text-davinci-003)
    \item Discourse-aware LMs (DMV)
    \item Word embeddings (GloVe)
    \item Structure representation (AMR+GCL, QA-SRL-ent).
    \item RelBERT \cite{ushio2021distilling}.
    \item LM Perplexities. Similar to \cite{ushio2021bert}, we develop specific prompts for LMs to obtain a perplexity score for a pair of stories.
\end{itemize}

(1) What contributes to the relational simiarity? 
SMT indicates the predicative feature contributes to the most relational similarity, is this true?

\input{floats/corr-results.tex}

\subsubsection{Supervised baselines}
Supervised retrieval methods:
\begin{itemize}
    \item Score-prediction. We finetuned RoBERTa/BERT models with an MLP to predict the entity similarity and relational similarity.
    \item Contrastive learning model. We conduct supervised contrastive learning using a triplet loss.
\end{itemize}



\subsubsection{Error analysis}
LMs cannot do? on which types ...




\subsection{Analogy generation}

If large language models can generate analogy pairs, can we transfer this ability to smaller language models via, e.g. finetuning or instruction tuning? And hence improving the innovative abilities afterwards? 
\textbf{Error analysis: LMs cannot do?}


\subsection{Problem solving by analogy retrieval}
\textbf{Doctor-tumor, General-fortresss}
We built a medium scale problem solving dataset based on the analogy data.
Specifically, the models are required to select one instance that is the most analogous to the target setting, and then make prediction.
Human evaluation is involved in solving the problems.
\textbf{Baselines}
\begin{itemize}
    \item Zero-shot prediction
    \item Few-shot, all candidates provided
    \item Few-shot, randomly sampled
    \item Few-shot, analogous retriever
\end{itemize}



\subsection{Extrinsic}

In this section, we aim to test how can the ability of analogy generalize to other domains.

\underline{Analogy and literal similarity} 
We know the difference of analogy and literal similarity through the discussion of SMT.
Intuitively, they are different in terms of topical similarity but not relational similarity. 
These data might serve as augmentation of training data to help model strengthen its understanding on the relational similarity.

We evaluate model performance on Semantic Textual Similarity (STS) tasks after finetuning it on our proposed benchmarks with contrastive learning paradigm.

\underline{Reasoning}
Ideally, using analogy can help model elicit similar (but not exactly the same) knowledge from its past memory. 
This could serves as important signal for reasoning tasks that requires intensive similarity knowledge.
To investigate this, we test how the analogy-aware models perform over natural language inference tasks (NLI).

\textbf{Doctor-tumor, general ...}

